Implicit Causal Representation Learning via Switchable Mechanisms

Learning causal representations from observational and interventional data in the absence of known ground-truth graph structures necessitates implicit latent causal representation learning. Implicit learning of causal mechanisms typically involves two categories of interventional data: hard and soft interventions. In real-world scenarios, soft interventions are often more realistic than hard interventions, as the latter require fully controlled environments. Unlike hard interventions, which directly force changes in a causal variable, soft interventions exert influence indirectly by affecting the causal mechanism. However, the subtlety of soft interventions impose several challenges for learning causal models. One challenge is that soft intervention's effects are ambiguous, since parental relations remain intact. In this paper, we tackle the challenges of learning causal models using soft interventions while retaining implicit modelling. We propose ICLR-SM, which models the effects of soft interventions by employing a causal mechanism switch variable designed to toggle between different causal mechanisms. In our experiments, we consistently observe improved learning of identifiable, causal representations, compared to baseline approaches.

==> figure1.tex <==
\begin{figure}[!h]
	\centering    
	\includegraphics[width=\textwidth]{figures/soft_ilcm_arc.pdf}
	\caption{~General overview of the SoftCD for learning an encoder, decoder, and solution function from interventional data. FC represents a fully connected neural network, and S the solution function. 
	\label{fig:model}}
\end{figure}


==> figure4.tex <==
\begin{figure}[!h]
	\centering
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{figures/baseline1.pdf}
		\caption{test}
		\label{fig:baseline1}
	\end{subfigure}
	\hspace{5em}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=0.3\textwidth]{figures/baseline2.pdf}
		\caption{}
		\label{fig:baseline2}
	\end{subfigure}
	\caption{Baseline Generative Models}
	\label{fig:baselines}
\end{figure}


==> figure8.tex <==
\begin{figure}[!h]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{graph_app1.pdf}
		\caption{}
		\label{fig:hard}
	\end{subfigure}
	\hspace{6em}
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{graph_app2.pdf}
		\caption{}
		\label{fig:soft}
	\end{subfigure}
	\caption{(a) String diagram of the causal variables $Z$ and $Z'$. The triangle indicates sampling $I$ from its distribution. The left-hand side diagram is when $\phi_{\mathcal{Z}}$ is applied last and the right-hand side diagram is when $\phi_{\mathcal{Z}}$ is applied first. $I$ is the intervention which affects intervened causal variable's mechanism variable. $V$ is used to model the effect of intervention on mechanisms and parents. (b) String diagrams after discarding $\Tilde{Z'_o}$ and the disentangled effect of soft intervention on $\Tilde{Z_i}$ modeled by $V$.}
	\label{fig:proof_soft_int}
\end{figure}



==> table3.tex <==

\begin{table}[!h]
    \centering
    \begin{small}
        \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{c c c c}
            \toprule
            \textbf{Edges} & \textbf{Post-intervention} & \textbf{Causal} & \textbf{Causal} \\
            & \textbf{causal mechanism} & \textbf{Disentanglement} & \textbf{Completeness} \\
            \midrule
            Chain & Default & 0.98 & 0.98 \\
            Full & Default & 0.89 & 0.89 \\
            Default & Significantly different & 0.68 & 0.73 \\
            Default & Almost similar & 0.85 & 0.86 \\  
            \bottomrule
        \end{tabular}
        }
        \caption{SoftCD performance on different configurations of $G5$}
        \label{tab:ablation}
    \end{small}
\end{table}






==> table5.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% TOP-K ACC %%%%%%%%%%%%%%%%%%%%%%%
%\begin{wraptable}{r}{0.5\textwidth}
\begin{table}[!h]
	\centering
	\caption{Action and object accuracy of three explicit models are compared with SoftCD. Experiments are conducted applying image with resolution of $R_{64}$ as the input to the Resnet50 encoder with the intervened casual variable ($z_i$).}
	\label{tab:explicit_softcd}
	\resizebox{7cm}{!}{
 \begin{small}
	\begin{tabular}{ll cc}
			\toprule
			\textbf{Datasets} & \textbf{Methods} & \textbf{Action Accuracy} & \textbf{Object Accuracy} \\
			\midrule
			Epic-Kitchens
			& ENCO \cite{enco}       &0.39      &0.07      \\
			& DDS \cite{dds}         &0.49      &0.09         \\
   			& Fixed-order        &0.34      &0.09         \\
			& \textbf{SoftCD (ours)}   &\textbf{0.63}      &\textbf{0.14} \\
            \midrule
            %\addlinespace
			ProcTHOR
			& ENCO \cite{enco}       &0.60       &0.64   \\
			& DDS \cite{dds}         &0.38       &0.44    \\
      		& Fixed-order        &0.43      &0.55         \\
			& \textbf{SoftCD (ours)}   &\textbf{0.75}       &\textbf{0.78}\\
   
			%\addlinespace   
			\bottomrule
	\end{tabular}
 \end{small}
 
 }
\end{table}
%\end{wraptable}



